Applied Nanofabrication for X-ray Grating Spectroscopy

Measuring the diffuse, highly-ionized baryonic content in galactic halos and the intergalactic medium through soft x-ray absorption spectroscopy of active galactic nuclei is a main scientific objective of the Lynx X-ray Observatory mission concept that can only be accomplished with a next-generation grating spectrometer. Realizing such an instrument using reflection grating technology requires thousands of custom blazed gratings that each perform with high diffraction efficiency to be manufactured and aligned to intercept radiation coming to a focus in a Wolter-I telescope. The aim of this thesis is to implement two recently-developed techniques in nanofabrication for this task, with an emphasis on beamline diffraction-efficiency testing for characterizing spectral sensitivity. In particular, thermally-activated selective topography equilibration (TASTE) is pursued as a means for fabricating a master grating with the key advantage that it enables blazed groove facets to be patterned in polymeric electron-beam resist over a non-parallel groove layout not limited by substrate crystal structure. Additionally, substrate-conformal imprint lithography (SCIL) is studied as a method for mass manufacturing high-fidelity grating replicas in a silica sol-gel resist while avoiding many of the detriments associated with large-area patterning in other nanoimprint techniques. Diffraction-efficiency testing of sub-micron grating prototypes coated with gold shows that TASTE is capable of meeting Lynx requirements for spectral sensitivity, with room for improvement at small groove periods, and that while SCIL offers a promising avenue for Lynx grating production, imprints suffer a small blaze-angle reduction due to resist shrinkage. Accompanying this dissertation are appendices that outline physics fundamentals for x-ray spectral lines, x-ray optics, and diffraction gratings.

==> SupplementaryMaterial/Dedication.tex <==
% Place the dedication below.
This dissertation is dedicated to my maternal great-grandmother, Edith Hatch Allen, my paternal grandfather, Richard Edward McCoy, and my maternal uncle, Jon Howard Hextell. 

==> SupplementaryMaterial/ListOfSymbols.tex <==
% Place the list of symbols below.
\begin{eqlist}[\def\makelabel#1{\hfill#1}\labelsep 1em]

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}

\item[$\alpha$]
The first greek letter, but we should really add some more text, though we need it to go on two lines, p.~\pageref{ChX-figure: FigureLabel7}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel4}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel5}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel6}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel7}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel8}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel9}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel10}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel4}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel5}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel6}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel7}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel8}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}

\item[$\alpha$]
The first greek letter, p.~\pageref{ChX-figure: FigureLabel3}

\end{eqlist}

==> SupplementaryMaterial/UserDefinedCommands.tex <==
% Place user-defined commands below.

% Define the \acro command.
\makeatletter
\newif\ifFirstPar       \FirstParfalse
\def\smc{\sc}
\def\ninepoint{\small}
\DeclareRobustCommand\SMC{%
  \ifx\@currsize\normalsize\small\else
   \ifx\@currsize\small\footnotesize\else
    \ifx\@currsize\footnotesize\scriptsize\else
     \ifx\@currsize\large\normalsize\else
      \ifx\@currsize\Large\large\else
       \ifx\@currsize\LARGE\Large\else
        \ifx\@currsize\scriptsize\tiny\else
         \ifx\@currsize\tiny\tiny\else
          \ifx\@currsize\huge\LARGE\else
           \ifx\@currsize\Huge\huge\else
            \small\SMC@unknown@warning
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
}
\newcommand\SMC@unknown@warning{\TBWarning{\string\SMC: unrecognised
    text font size command -- using \string\small}}
\newcommand\textSMC[1]{{\SMC #1}}
\newcommand\acro[1]{\textSMC{#1}\@}

\makeatother

% command for vectors
\newcommand{\bv}[1]{\ensuremath{\vec{#1}}}
% command for unit vectors
\newcommand{\uv}[2][blank]{%
\ifthenelse{\equal{#1}{blank}}%
{\ensuremath{\hat{u}_{#2}}}%
{}%
%
\ifthenelse{\equal{#1}{.}}%
{\ensuremath{\dot{\hat{u}}_{#2}}}%
{}%
%
\ifthenelse{\equal{#1}{'}}%
{\ensuremath{\hat{u}'_{#2}}}%
{}%
}
\newcommand{\ui}{\ensuremath{\hat{\imath}}}
\newcommand{\uj}{\ensuremath{\hat{\jmath}}}
\newcommand{\uk}{\ensuremath{\hat{k}}}

\newcommand\ion[2]{#1$\;${\scshape{#2}}}%                       % ion, i.e., CII = \ion{C}{ii}


==> eqparbox/README <==
                  +--------------------------------+
                  |EQPARBOX: Equal-widthed parboxes|
                  |By Scott Pakin <pakin@uiuc.edu> |
                  +--------------------------------+


Description
-----------

LaTeX users sometimes need to ensure that two or more blocks of text
occupy the same amount of horizontal space on the page.  To that end,
the eqparbox package defines a new command, \eqparbox, which works
just like \parbox, except that instead of specifying a width, one
specifies a tag.  All eqparboxes with the same tag -- regardless of
where they are in the document -- will stretch to fit the widest
eqparbox with that tag.  This simple, equal-width mechanism can be
used for a variety of alignment purposes, as is evidenced by the
examples in eqparbox's documentation.


Installation
------------

There's nothing special about building eqparbox:

    latex eqparbox.ins     <== Generate eqparbox.sty
    latex eqparbox.dtx     <== Produce the documentation (eqparbox.dvi)
    latex eqparbox.dtx     <== Again, to get labels and eqparboxes right
    makeindex -s gind.ist eqparbox    <== Generate an index
    latex eqparbox.dtx     <== Incorporate the index into the document

If you're new to this, see
http://www.tex.ac.uk/cgi-bin/texfaq2html?label=instpackages for more
information on installing packages.


Copyright and license
---------------------
Copyright (C) 2001 Scott Pakin <pakin@uiuc.edu>

This package may be distributed and/or modified under the conditions
of the LaTeX Project Public License, either version 1.2 of this
license or (at your option) any later version.  The latest version of
this license is in:

    http://www.latex-project.org/lppl.txt

and version 1.2 or later is part of all distributions of LaTeX version
1999/12/01 or later.

